Zero-shot Singing Technique Conversion

In this paper we propose modifications to the neural network framework, AutoVC for the task of singing technique conversion. This includes utilising a pretrained singing technique encoder which extracts technique information, upon which a decoder is conditioned during training. By swapping out a source singer's technique information for that of the target's during conversion, the input spectrogram is reconstructed with the target's technique. We document the beneficial effects of omitting the latent loss, the importance of sequential training, and our process for fine-tuning the bottleneck. We also conducted a listening study where participants rate the specificity of technique-converted voices as well as their naturalness. From this we are able to conclude how effective the technique conversions are and how different conditions affect them, while assessing the model's ability to reconstruct its input data.

==> 09-Bibfile.tex <==
\begin{thebibliography}{4}

\bibitem{jour} Smith, T.F., Waterman, M.S.: Identification of Common Molecular
Subsequences. J. Mol. Biol. 147, 195--197 (1981)

\bibitem{lncschap} May, P., Ehrlich, H.C., Steinke, T.: ZIB Structure Prediction Pipeline:
Composing a Complex Biological Workflow through Web Services. In: Nagel,
W.E., Walter, W.V., Lehner, W. (eds.) Euro-Par 2006. LNCS, vol. 4128,
pp. 1148--1158. Springer, Heidelberg (2006)

\bibitem{book} Foster, I., Kesselman, C.: The Grid: Blueprint for a New Computing
Infrastructure. Morgan Kaufmann, San Francisco (1999)

\bibitem{proceeding1} Czajkowski, K., Fitzgerald, S., Foster, I., Kesselman, C.: Grid
Information Services for Distributed Resource Sharing. In: 10th IEEE
International Symposium on High Performance Distributed Computing, pp.
181--184. IEEE Press, New York (2001)

\bibitem{proceeding2} Foster, I., Kesselman, C., Nick, J., Tuecke, S.: The Physiology of the
Grid: an Open Grid Services Architecture for Distributed Systems
Integration. Technical report, Global Grid Forum (2002)

\bibitem{url} National Center for Biotechnology Information, \url{http://www.ncbi.nlm.nih.gov}

\bibitem{basak2021a} Basak, S., Agarwal, S., Ganapathy, S., Takahashi, N.: End-to-end Lyrics Recognition with Voice to Singing Style Transfer. In: 2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), pp. 266–270 (2021) https://doi.org/10.1109/ICASSP39728.2021.9415096

\bibitem{bittner2014} Bittner, R., Salamon, J., Tierney, M., Mauch, M., Cannam,  C., Bello, J.: MedleyDB: A Multitrack Dataset for Annotation-intensive MIR Research. In: 15th International Society for Music Information Retrieval Conference, pp. 155--160. (2014)

\bibitem{chandna2020} Chandna, P., Blaauw, M., Bonada, J., Gomez, E: Content Based Singing Voice Extraction from a Musical Mixture. In: 2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), pp. 781-785 (2020)

\bibitem{choi2017} Choi, K., Fazekas, G., Sandler, M., Cho, K.: Convolutional Recurrentneural Networks for Music Classification. In: 2017 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), pp. 2392–2396. (2017) \url{https://doi.org/10.1109/ICASSP.2017.7952585}

\bibitem{heidemann2016} Heidemann, K.: A System for Describing Vocal Timbre in Popular Pong. In: Music Theory Online, vol. 22, (2016) \url{https://doi.org/10.30535/mto.22.1.2}

\bibitem{hsu2019} Hsu, W.-N., Zhang, Y., Weiss, R. J., Zen, H., Wu, Y., Wang, Y., Pang, R.: Hierarchical Generative Modeling for Controllable Speech Synthesis. In: The International Conference on Learning Representations, p. 27. New Orleans, LA, USA (2019)

\bibitem{jillings2015} Jillings, N., Moffat, D., De Man, B., Reiss, J. D.: Web Audio Evaluation Tool: A  browse-based  listening  environment. In: 12th Sound and Music Computing Conference. Maynooth, Ireland. (2015)

\bibitem{lee2019} Lee, J., Choi, H.-S., Jeon, C.-B., Koo, J., Lee, K.: Adversarially Trained End-to-end Korean Singing Voice Synthesis System. arXic preprint arXiv:1908.01919 (2019)

\bibitem{lee2020} Lee, J., Choi, H.-S., Koo, J., Lee, K.: Disentangling Timbre and Singing Style with Multi-Singer Singing Synthesis System. In: 2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), pp. 7224–7228 (2020) \url{https://doi.org/10.1109/ICASSP40776.2020.9054636}

\bibitem{luo2019} Luo, Y.-J., Hsu, C.-C., Agres, K., Herremans, D.: (2019). Singing Voice Conversion with Disentangled Representations of Singer and Vocal Technique Using Variational Autoencoders. arXiv preprint arXiv:1912.02613 (2019)

\bibitem{meseguer-brocal2020} Meseguer-Brocal, G., Cohen-Hadria, A., Peeters, G.: Creating DALI,a  Large  Dataset  of  Synchronized  Audio,  Lyrics,  and  Notes. In: Transactions of the International Society for Music Information Retrieval, vol. 3 pp. 55-67 (2020) https://doi.org/10.5334/tismir.30

\bibitem{nachmani2019} Nachmani, E., Wolf, L.: Unsupervised Singing Voice Conversion. arXiv preprint arXiv:1904.06590 (2019)

\bibitem{nercessian2020} Nercessian, S.: Zero-shot Singing Voice Conversion.  In: Proceedings of the International Society for Music Information Retrieval Conference (2020)

\bibitem{oconnor2020} O’Connor, B., Dixon, S., Fazekas, G.: An Exploratory Study on Perceptual Spaces of the Singing Voice. In: The 2020 Joint AI Conference on Music Creativity, vol. 1, Stockholm, Sweden (2020)

\bibitem{jia2019} Jia, Y., Zhang, Y., Weiss, R. J., Wang, Q., Shen, J., Ren, F., Wu, Y.: Transfer  Learning  from  Speaker  Verification  to  Multispeaker  Text-To-Speech Synthesis. arXiv preprint arXiv:1806.04558 (2019)

\bibitem{qian2019} Qian, K., Zhang, Y., Chang, S., Yang, X., Hasegawa-Johnson, M.: AutoVC: Zero-Shot Voice Style Transfer with Only Autoencoder Loss. In: 36th International Conference of Machine Learning, vol. 47, pp. 5210-5219 (2019)

\bibitem{qian2020} Qian, K., Jin, Z., Hasegawa-Johnson, M., Mysore, G. J.: F0-Consistent  Many-To-Many  Non-Parallel  Voice  Conversion  Via  Conditional Autoencoder. In: 2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), pp. 6284–6288 (2020) \url{https://doi.org/10.1109/ICASSP40776.2020.9054734}

\bibitem{qian2020a} Qian, K., Zhang, Y., Chang, S., Cox, D., Hasegawa-Johnson, M.: Unsupervised speech decomposition via triple information bottleneck. In: 37th International Conference on Machine Learning, vol. 119, pp. 7792–7802 (2020)

\bibitem{raffel2016} Raffel, C., Ellis, D. P. W.: Feed-Forward Networks with Attention Can Solve Some Long-Term Memory Problems. arXiv preprint arXiv:1512.08756 (2016)

\bibitem{ronneberger2015} Ronneberger, O., Fischer, P., Brox, T: U-Net: Convolutional Networks for Biomedical Image Segmentation. In: N. Navab, J. Hornegger, W. M. Wells, A. F. Frangi (eds.) Medical Image Computing and Computer-Assisted Intervention, vol. 9351, pp. 234–241. (2015) \url{https://doi.org/10.1007/978-3-319-24574-428}

\bibitem{tolstikhin2019} Tolstikhin, I., Bousquet, O., Gelly, S., Schoelkopf, B.: Wasserstein Auto-Encoders. arXiv preprint arXiv:1711.01558 (2019)

\bibitem{veaux2017} Veaux, C., Yamagishi, J., MacDonald, K.: CSTR VCTK Corpus: English multi-speaker Corpus for CSTR Voice Cloning Toolkit. (2017) \url{https://doi.org/10.7488/ds/2645}

\bibitem{wan2018} Wan, L., Wang, Q., Papir, A., Moreno, I. L.: Generalized End-to-End Loss for Speaker Verification. In: 2018 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), pp. 4879–4883 (2018) \url{https://doi.org/10.1109/ICASSP.2018.8462665}

\bibitem{wilkins2018} Wilkins, J., Seetharaman, P., Wahl, A., Pardo, B. (2018).: VocalSet: A Singing Voice Dataset. 19th International Society for Music Information Retrieval Conference, Paris ,France pp. 468--474 (2018)

\bibitem{wu2020} Wu, D.Y., Chen, Y.H., Lee, H.Y.: One-Shot Voice Conversion by Vector Quantization. In: 2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP) (2020)

\end{thebibliography}
